Multi-Resolution Continuous Normalizing Flows

Recent work has shown that Neural Ordinary Differential Equations (ODEs) can serve as generative models of images using the perspective of Continuous Normalizing Flows (CNFs). Such models offer exact likelihood calculation, and invertible generation/density estimation. In this work we introduce a Multi-Resolution variant of such models (MRCNF), by characterizing the conditional distribution over the additional information required to generate a fine image that is consistent with the coarse image. We introduce a transformation between resolutions that allows for no change in the log likelihood. We show that this approach yields comparable likelihood values for various image datasets, with improved performance at higher resolutions, with fewer parameters, using only 1 GPU. Further, we examine the out-of-distribution properties of (Multi-Resolution) Continuous Normalizing Flows, and find that they are similar to those of other likelihood-based generative models.

==> text/fig_bpd.tex <==
\begin{figure*}[thb]
     \centering
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/1sc.png}
         \caption{1-resolution}
         \label{fig:1sc}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.26\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/2sc.png}
         \caption{2-resolution}
         \label{fig:2sc}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.26\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/3sc.png}
         \caption{3-resolution}
         \label{fig:3sc}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.26\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/4sc.png}
         \caption{4-resolution}
         \label{fig:4sc}
     \end{subfigure}
    \caption{\small{Bits-per-dim vs Epoch at each resolution for different \gls{msflow-image} models (FFJORD RNODE) trained on CIFAR10.}}
    \label{fig:bpds}
    \vspace{-0.5em}
\end{figure*}


==> text/fig_mrcnf_1d_gen.tex <==
\begin{figure}[!hb]
\vspace{-.25cm}
\begin{center}
\includegraphics[width=0.75\linewidth]{figs/MRCNF4_1d_GEN.png}
\end{center}
\caption{The architecture of our \gls{msflow-image} method. Normalizing flows are used to generate images at each resolution, with finer resolutions being generated conditioned on the coarser image one level above.}
\label{fig:mrcnf_1d_gen}
\end{figure}

==> text/fig_mrcnf_train.tex <==
\begin{figure}[!hb]
\vspace{-.25cm}
\begin{center}
\includegraphics[width=0.72\linewidth]{figs/MRCNF5_TRAIN.png}
\end{center}
\caption{The architecture of our \gls{msflow-image} method. Normalizing flows are used to generate images at each resolution, with finer resolutions being generated conditioned on the coarser image one level above.}
\label{fig:mrcnf_train}
\end{figure}

==> text/fig_msflow_image.tex <==
\begin{figure}[!hb]
\vspace{-.25cm}
\begin{center}
\includegraphics[width=0.72\linewidth]{figs/MSFLOW_Image.png}
\end{center}
\caption{The architecture of our \gls{msflow-image} method. Normalizing flows are used to generate images at each resolution, with finer resolutions being generated conditioned on the coarser image one level above.}
\label{fig:msflow-image}
\end{figure}

==> text/figtable.tex <==
\begin{figure}[h]
\begin{minipage}[t]{0.45\linewidth}
\centering
% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=\linewidth]{figs/MRCNF_OOD.png}
\caption{\small{Histogram of log likelihood per dimension of out-of-distribution datasets (TinyImageNet, SVHN, Constant images) under (MR)CNF models trained on CIFAR10. As with other likelihood-based generative models such as Glow \& PixelCNN, OoD datasets have higher likelihood under (MR)CNFs.}}
\label{fig:ood_bpd_A}
\end{minipage}
\end{figure}


==> text/table1_OLD_params_bpd_time_OLD.tex <==
\begin{table*}[!htb]
    \small
    \centering
    \begin{tabular}{|l@{\hskip -2em}|ccc|ccc|ccc|}
        \hline
        % & \multicolumn{3}{|c|}{MNIST}
        & \multicolumn{3}{c|}{\textbf{\textsc{CIFAR10}}} & \multicolumn{3}{c|}{\textbf{\textsc{ImageNet32}}} & \multicolumn{3}{c|}{\textbf{\textsc{ImageNet64}}} \\
        & \textsc{Param}
        & \textsc{BPD} 
        & \textsc{Time}
        % & \begin{tabular}{@{}c@{}}Time \\ (Hours)\end{tabular}
        % & \begin{tabular}{@{}c@{}}Time/100 \\ Epochs\end{tabular}
        % & Time
        & \textsc{Param} & \textsc{BPD} & \textsc{Time}
        & \textsc{Param} & \textsc{BPD} & \textsc{Time} \\
        \hline\hline
        \multicolumn{10}{|l|}{\textbf{Non Flow-based Prior Work}} \\
        \hline
        PixelRNN~\cite{oord2016pixel} 
            &  & 3.00 & 
            &  & 3.86 & 
            &  & 3.63 & \\[-2pt]
        % NeurIPS 2016
        Gated PixelCNN
        ~\cite{van2016conditional}
        % (32 GPUs)
            % &  & & 
            &  & 3.03 & 
            &  & 3.83 & 60
            &  & 3.57 & 60 \\[-2pt]
        % ICLR 2017
        Parallel Multiscale
        ~\cite{reed2017parallel}
            % &  & & 
            &  &  & 
            &  & 3.95 & 
            &  & 3.70 &  \\[-2pt]
        % ICML 2018
        Image Transformer
        ~\cite{parmar2018image}
            % &  & & 
            &  & 2.90 & 
            &  & 3.77 &  
            &  &  &   \\[-2pt]
        % ICML 2018
        PixelSNAIL
        ~\cite{chen2018pixelsnail}
            % &  & & 
            &  & 2.85 & 
            &  & 3.80 &  
            &  &  &   \\[-2pt]
        % ICLR 2019
        SPN
        ~\cite{menick2019generating}
            % &  & & 
            &  &  & 
            & \footnotesize{150M} & 3.85 &  
            & \footnotesize{150M} & 3.53 &   \\[-2pt]
        % 2019
        Sparse Transformer
        ~\cite{child2019generating}
            % &  & & 
            & \footnotesize{59M} & 2.80 & 
            &  &  &  
            & \footnotesize{152M} & 3.44 & \footnotesize{7days}  \\[-2pt]
        % 2019
        Axial Transformer
        ~\cite{ho2019axial}
            % &  & & 
            &  &  & 
            &  & 3.76 &  
            &  & 3.44 &   \\[-2pt]
        % NeurIPS 2020
        PixelFlow++
        ~\cite{nielsen2020closing}
            % & ? & &
            &  & 2.92 &
            &  &  & 
            &  &  &  \\[-2pt]
        % NeurIPS 2020
        NVAE
        ~\cite{vahdat2020nvae}
            % &  & & 
            &  & 2.91 & 55
            &  & 3.92 & 70 
            &  &  &   \\[-2pt]
        % ICML 2020
        Dist-Aug Sparse Transformer
        ~\cite{jun2020distaug}
            % & & 
            & \footnotesize{152M} & 2.56 &
            &  &  & 
            & \footnotesize{152M} & 3.42 &  \\
        % % 2020
        % Denoising
        % % ~\cite{ho2020denoising}
        %     &  & &
        %     &  & &
        %     &  & 3.75 &
        %     &  & & \\
        \hline
        \hline
        \multicolumn{10}{|l|}{\textbf{Flow-based Prior Work}} \\
        \hline
        % % ICML 2015
        % Diffusion
        % % ~\cite{sohl2015deep}
        %     & & 1.34 &
        %     & & 5.4 &
        %     &  &  & 
        %     &  &  &  \\
        % % NeurIPS 2016
        % IAF
        % % ~\cite{kingma2016improved}
        %     &  &  & 
        %     & & 3.11 &
        %     &  &  & 
        %     &  &  &  \\
        % ICLR 2017
        RealNVP
        ~\cite{dinh2016density}
            % & & 1.06 &
            & & 3.49 & 
            & \footnotesize{46.0M} & 4.28 & 
            & \footnotesize{96.0M} & 3.98 & \\[-2pt]
        % NeurIPS 2018
        Glow
        ~\cite{kingma2018glow}
            % & & 1.05 &
            & \footnotesize{44.0M} & 3.35 &
            & \footnotesize{66.1M} & 4.09 & 
            & \footnotesize{111.1M} & 3.81 & \\[-2pt]
        % % ICML 2019
        % i-ResNets
        % ~\cite{behrmann2019invertible}
        %     % & & 1.05 &
        %     &  &  & 
        %     &  &  &  
        %     &  &  &  \\[-2pt]
        % ICML 2019
        Emerging
        ~\cite{hoogeboom2019emerging}
            % &  &  & 
            & \footnotesize{44.7M} & 3.34 &
            & \footnotesize{67.1M} & 4.09 &
            & \footnotesize{67.1M} & 3.81 & \\[-2pt]
        % NeurIPS 2019
        IDF
        ~\cite{hoogeboom2019idf}
            % &  &  & 
            & & 3.34 &
            & & 4.18 &
            & & 3.90 & \\[-2pt]
        % NeurIPS 2019
        S-CONF
        ~\cite{karami2019invertible}
            % &  &  & 
            & & 3.34 &
            & & &
            & & & \\[-2pt]
        % NeurIPS 2019
        MintNet
        ~\cite{song2019mintnet}
            % &  &  & 
            & \footnotesize{17.9M} & 3.32 & \footnotesize{$\geq$5days}
            & \footnotesize{17.4M} & 4.06 &
            &  &  &  \\[-2pt]
        % NeurIPS 2019
        Residual Flow
        ~\cite{chen2019residual}
            % &  &  & 
            & & 3.28 &
            & & 4.01 &
            & & 3.76 & \\[-2pt]
        % NeurIPS 2019
        MaCow
        ~\cite{ma2019macow}
            % &  &  & 
            & 43.5M & 3.16 &
            &  &  & 
            & 122.5M & 3.69 & \\[-2pt]
        % NeurIPS 2019
        Neural Spline Flows
        ~\cite{durkan2019spline}
            % &  &  & 
            & \footnotesize{11.8M} & 3.38 &
            & & &
            & \footnotesize{15.6M} & 3.82 & \\[-2pt]
        % ICML 2019
        Flow++
        ~\cite{ho2019flow++}
            % &  &  & 
            & \footnotesize{31.4M} & 3.08 &
            & \footnotesize{169M} & 3.86 &
            & \footnotesize{73.5M} & 3.69 & \\[-2pt]
        % 2020
        ANF
        ~\cite{huang2020augmented}
            % &  &  & 
            &  & 3.05 &
            &  & 3.92 &
            &  & 3.66 & \\[-2pt]
        % ICML 2020
        MEF
        ~\cite{xiao2020generative}
            % &  &  & 
            & \footnotesize{37.7M} & 3.32 &
            & \footnotesize{37.7M} & 4.05 &
            & \footnotesize{46.6M} & 3.73 & \\[-2pt]
        % ICML 2020
        VFlow
        ~\cite{chen2020vflow}
            % &  &  & 
            &  & 2.98 & 
            &  & 3.83 & 
            &  &  &   \\[-2pt]
        % % NeurIPS 2020
        % Woodbury NF
        % ~\cite{lu2020woodbury}
        %     % &  &  & 
        %     & & 3.47 & 
        %     & & 4.20 & 
        %     & & 3.87 &  \\
        % % NeurIPS 2020
        % NanoFlow
        % ~\cite{lee2020nanoflow}
        %     % &  & & 
        %     &  & 3.25 & 
        %     &  &  &  
        %     &  &  &   \\
        % % NeurIPS 2020
        % Convolution Exponential
        % ~\cite{hoogeboom2020flow}
        %     % &  & &
        %     &  & 3.218 &
        %     &  &  & 
        %     &  &  &  \\
        % NeurIPS 2020
        Wavelet Flow
        ~\cite{yu2020waveletflow}
            % &  & & 
            &  &  & 
            & \footnotesize{64M} & 4.08 & 
            & \footnotesize{96M} & 3.78 & 822  \\
        % % 2020
        % TayNODE
        % % ~\cite{kelly2020learning}
        %     &  & 1.039 & 
        %     &  & & 
        %     &  & &  \\
        \hline
        \hline
        \multicolumn{10}{|l|}{\textbf{1-resolution Continuous Normalizing Flow}}\\
        \hline
        % ICLR 2019
        FFJORD
        ~\cite{grathwohl2019ffjord}
            % & 0.99 & &
            & \multirow{4}{*}{\footnotesize{1.36M}} & 3.40 & \footnotesize{$\geq$5days}
            & \multirow{4}{*}{\footnotesize{2.00M}} & $3.96^{\ddagger}$ & \footnotesize{$>$5days$^{\ddagger}$}
            & \multirow{4}{*}{\footnotesize{2.00M}} & x & x \\[-2pt]
        % % ICML 2020
        % FFJORD, \textsc{vanilla}
        % % ~\cite{finlay2020train}
        %     % & 0.97 & 68.5 
        %     & 3.36 & & 91.3 
        %     & ?? & ??
        %     & x & x \\
        % ICML 2020
        FFJORD RNODE
        ~\cite{finlay2020rnode}
            % & 0.97 & 24.4 &
            & & 3.38 & 31.84
            & & $2.36^{\ddagger}$ & $30.1^{\ddagger}$
            & & $3.83^*$ & $64.1^*$ \\[-2pt]
        % NeurIPS 2020
        FFJORD + STEER
        ~\cite{ghosh2020steer}
            % & 0.974 & 51.21 &
            & & 3.40 & 86.34
            & & 3.84 & \footnotesize{$>$5days}
            & & & \\[-2pt]
        % NeurIPS 2020
        FFJORD RNODE + STEER
        ~\cite{ghosh2020steer}
            & & 3.397 & 22.24
            & & 2.35 & 24.9
            & & & \\
        \hline
        \hline
        \multicolumn{10}{|l|}{\textbf{\textsc{(Ours)} 2-resolution \gls{msflow-image}}}\\
        \hline
        2res FFJORD
            % & ?? & ??
            & \multirow{4}{*}{\footnotesize{0.48M}}
            & 1.85 & 17.89 
            & \multirow{4}{*}{\footnotesize{0.16M}}
            & x & x
            & \multirow{4}{*}{\footnotesize{0.16M}}
            & x & x \\[-2pt]
        2res FFJORD RNODE
            % & ?? & ??
            & & \textbf{1.69} & 16.37 
            & & \textbf{1.92} & 26.20 
            & & \textbf{1.54} & 51.21  \\[-2pt]
        2res FFJORD + STEER
            % & ?? & ??
            & & 2.04 & 18.76 
            & & 2.36 & 20.12 
            & & x & x \\[-2pt]
        2res FFJORD RNODE + STEER
            % & ?? & ??
            & & 1.74 & 18.43 
            & & 1.97 & 65.16 
            & & 1.58 & 66.76  \\
        \hline
        \hline
        \multicolumn{10}{|l|}{\textbf{\textsc{(Ours)} 3-resolution \gls{msflow-image}}}\\
        \hline
        3res FFJORD
            % & ?? & ?? 
            & \multirow{4}{*}{\footnotesize{0.48M}} & 1.54 & 21.51
            & \multirow{4}{*}{\footnotesize{0.13M}} & 2.00 & 30.54
            & \multirow{4}{*}{\footnotesize{0.13M}} & x & x  \\[-2pt]
        3res FFJORD RNODE
            % & ?? & ??
            & & \textbf{1.32} & 21.48
            & & \textbf{1.66} & 41.17
            & & \textbf{1.21}  & 60.89 \\[-2pt]
        3res FFJORD + STEER
            % & & ?? & ?? 
            & & 1.72 & 21.09 
            & & 2.21 & 21.36 
            & & x & x  \\[-2pt]
        3res FFJORD RNODE + STEER
            % & & ?? & ?? 
            & & 1.44 & 23.44 
            & & 1.68 & 54.05 
            & & 1.26 & 59.14  \\
        \hline
        \hline
        \multicolumn{10}{|l|}{\textbf{\textsc{(Ours)} 4-resolution \gls{msflow-image}}}\\
        \hline
        4res FFJORD
            % & & ?? & ?? 
            & \multirow{4}{*}{\footnotesize{0.64M}} & 1.42 & 19.95 
            & \multirow{4}{*}{\footnotesize{0.17M}} & 1.84 & 30.63 
            & \multirow{4}{*}{\footnotesize{0.17M}} & x & x \\[-2pt]
        4res FFJORD RNODE
            % & & ?? & ?? 
            & & \textbf{1.28} & 19.08 
            & & \textbf{1.62} & 42.60 
            & & \textbf{1.18} & 65.6  \\[-2pt]
        4res FFJORD + STEER
            % & & ?? & ??
            & & 1.88 & 17.73
            & & x & x 
            & & x & x \\[-2pt]
        4res FFJORD RNODE + STEER
            % & & ?? & ?? & ??
            & & 1.44 & 17.60
            & & 1.63 & 62.82
            & & 1.36 & 66.2 \\
        \hline
        \hline
        \textbf{\textsc{(Ours)} 5-resolution \gls{msflow-image}}
        & \footnotesize{0.81M} & \textbf{1.28} & 19.42
        & \footnotesize{} & &
        & \footnotesize{0.22M} & \textbf{1.17} & 71.33 \\
        \textbf{\textsc{(Ours)} 6-resolution \gls{msflow-image}} 
        & \footnotesize{0.97M} & \textbf{1.24} & 20.52
        & \footnotesize{} & &
        & \footnotesize{} & & \\
        \hline
        \hline
        \textbf{\textsc{(Ours)} 2-resolution \gls{msflow-wv}}
        & \footnotesize{0.50M} & 3.56 & 17.17
        & \footnotesize{0.33M} & 3.92 & 15.30
        & \footnotesize{} & & \\
        \textbf{\textsc{(Ours)} 3-resolution \gls{msflow-wv}} 
        & \footnotesize{0.76M} & 3.69 & 13.99
        & \footnotesize{0.51M} & 4.00 & 17.70
        & \footnotesize{0.51M} & 4.04 & 37.82 \\
        \textbf{\textsc{(Ours)} 4-resolution \gls{msflow-wv}} 
        & \footnotesize{1.03M} & 3.77 & 13.94
        & \footnotesize{0.69M} & 4.02 & 16.83
        & \footnotesize{} &  & \\
        \textbf{\textsc{(Ours)} 5-resolution \gls{msflow-wv}} 
        & \footnotesize{1.29M} & 3.87 & 10.73
        & \footnotesize{} &  & 
        & \footnotesize{} &  & \\
        \hline
    \end{tabular}
    \caption{\normalsize{Unconditional image generation metrics (lower is better in all cases): number of parameters in the model, bits-per-dimension, time (in hours). Check Tables~\ref{tab:msflow_cifar}, ~\ref{tab:msflow_wavelet} for a more detailed report. Most previous models use multiple GPUs for training, all our models were trained on only \textit{one} NVIDIA V100 GPU.
    % $^\dagger$As reported in~\cite{chen2019residual}.
    $^\ddagger$As reported in~\cite{ghosh2020steer}.
    % $^{\#}$Unreported in original paper, computed by us.
    $^*$FFJORD RNODE~\cite{finlay2020rnode} used 4 GPUs to train on ImageNet64. `x': Fails to train.}}
    \label{tab:msflow}
    % \vspace{-1.5em}
\end{table*}


==> text/table1_params_bpd_time.tex <==
\begin{table*}[!htb]
    \small
    \centering
    {\def\arraystretch{1.1}
    \setlength{\tabcolsep}{.15em}   \caption{\normalsize{Bits-per-dimension (lower is better) of images in the corresponding evaluation sets for CIFAR10, ImageNet at $32\x32$, and ImageNet at $64\x64$, reported as the mean and standard deviation across the dataset. We also report the number of parameters in the models, and the time taken to train (in GPU hours). Most previous models use multiple GPUs for training, all our models were trained on only \textit{one} GPU: NVIDIA RTX 2080 Ti with 11GB.\\
    Blank spaces indicate unreported values.
    % $^\dagger$As reported in~\cite{chen2019residual}.
    \quad
    $^\ddagger$As reported in~\cite{ghosh2020steer}. \quad `x': Fails to train.\\ $^\mathsection$Re-implemented by us.
    \quad
    $^*$RNODE~\cite{finlay2020rnode} used 4 GPUs to train on ImageNet64.}}
    \begin{tabular}{|l|ccc|ccc|ccc|}
        \hline
        % & \multicolumn{3}{|c|}{MNIST}
        & \multicolumn{3}{c|}{\textbf{\textsc{CIFAR10}}} & \multicolumn{3}{c|}{\textbf{\textsc{ImageNet32}}} & \multicolumn{3}{c|}{\textbf{\textsc{ImageNet64}}} \Tstrut \\
        & \textsc{BPD} & \textsc{Param} & \textsc{Time}
        % & \begin{tabular}{@{}c@{}}Time \\ (Hours)\end{tabular}
        % & \begin{tabular}{@{}c@{}}Time/100 \\ Epochs\end{tabular}
        % & Time
        & \textsc{BPD} & \textsc{Param} & \textsc{Time}
        & \textsc{BPD} & \textsc{Param} & \textsc{Time} \\
        \hline\hline
        \multicolumn{10}{|l|}{\textbf{Non Flow-based Prior Work}} \Tstrut \\
        \hline
        PixelRNN~\cite{oord2016pixel} 
            & 3.00 & & 
            & 3.86 & & 
            & 3.63 & & \\[-2pt]
        % NeurIPS 2016
        Gated PixelCNN
        ~\cite{van2016conditional}
        % (32 GPUs)
            % &  & & 
            & 3.03 &  & 
            & 3.83 &  & 60
            & 3.57 &  & 60 \\[-2pt]
        % ICLR 2017
        Parallel Multiscale
        ~\cite{reed2017parallel}
            % &  & & 
            & & & 
            & 3.95 & & 
            & 3.70 & &  \\[-2pt]
        % ICML 2018
        Image Transformer
        ~\cite{parmar2018image}
            % &  & & 
            & 2.90 &  & 
            & 3.77 &  &  
            &  &  &   \\[-2pt]
        % ICML 2018
        PixelSNAIL
        ~\cite{chen2018pixelsnail}
            % &  & & 
            & 2.85 &  & 
            & 3.80 &  &  
            &  &  &   \\[-2pt]
        % ICLR 2019
        SPN
        ~\cite{menick2019generating}
            % &  & & 
            &  &  & 
            & 3.85 & \footnotesize{150M} &  
            & 3.53 & \footnotesize{150M} &   \\[-2pt]
        % 2019
        Sparse Transformer
        ~\cite{child2019generating}
            % &  & & 
            & 2.80 & \footnotesize{59M} & 
            &  &  &  
            & 3.44 & \footnotesize{152M} & \footnotesize{7days}  \\[-2pt]
        % 2019
        Axial Transformer
        ~\cite{ho2019axial}
            % &  & & 
            &  &  & 
            & 3.76 &  &  
            & 3.44 &  &   \\[-2pt]
        % NeurIPS 2020
        PixelFlow++
        ~\cite{nielsen2020closing}
            % & ? & &
            & 2.92 &  &
            &  &  & 
            &  &  &  \\[-2pt]
        % NeurIPS 2020
        NVAE
        ~\cite{vahdat2020nvae}
            % &  & & 
            & 2.91 &  & 55
            & 3.92 &  & 70 
            &  &  &   \\[-2pt]
        % ICML 2020
        DistAug
        ~\cite{jun2020distaug}
            % & & 
            & 2.56 & \footnotesize{152M} &
            &  &  & 
            & 3.42 & \footnotesize{152M} &  \\
        % % 2020
        % Denoising
        % % ~\cite{ho2020denoising}
        %     &  & &
        %     &  & &
        %     & $\leq$ 3.75 & &
        %     &  & & \\
        \hline
        \hline
        \multicolumn{10}{|l|}{\textbf{Flow-based Prior Work}} \Tstrut \\
        \hline
        % % ICML 2015
        % Diffusion
        % % ~\cite{sohl2015deep}
        %     & 1.34 & &
        %     & 5.4 & &
        %     &  &  & 
        %     &  &  &  \\[-2pt]
        % % NeurIPS 2016
        % IAF
        % % ~\cite{kingma2016improved}
        %     &  &  & 
        %     & 3.11 & &
        %     &  &  & 
        %     &  &  &  \\[-0pt]
        % ICLR 2017
        RealNVP
        ~\cite{dinh2016density}
            % & & 1.06 &
            & 3.49 & & 
            & 4.28 & \footnotesize{46.0M} & 
            & 3.98 & \footnotesize{96.0M} & \\[-2pt]
        % NeurIPS 2018
        Glow
        ~\cite{kingma2018glow}
            % & & 1.05 &
            & 3.35 & \footnotesize{44.0M} &
            & 4.09 & \footnotesize{66.1M} & 
            & 3.81 & \footnotesize{111.1M} & \\[-2pt]
        % % ICML 2019
        % i-ResNets
        % ~\cite{behrmann2019invertible}
        %     % & 1.05 & &
        %     &  &  & 
        %     &  &  &  
        %     &  &  &  \\[-2pt]
        % % ICML 2019
        % Emerging
        % ~\cite{hoogeboom2019emerging}
        %     % &  &  & 
        %     & 3.34 & \footnotesize{44.7M} &
        %     & 4.09 & \footnotesize{67.1M} &
        %     & 3.81 & \footnotesize{67.1M} & \\[-2pt]
        % % NeurIPS 2019
        % IDF
        % ~\cite{hoogeboom2019idf}
        %     % &  &  & 
        %     & 3.34 & &
        %     & 4.18 & &
        %     & 3.90 & & \\[-2pt]
        % % NeurIPS 2019
        % S-CONF
        % ~\cite{karami2019invertible}
        %     % &  &  & 
        %     & 3.34 & &
        %     & & &
        %     & & & \\[-2pt]
        % NeurIPS 2019
        MintNet
        ~\cite{song2019mintnet}
            % &  &  & 
            & 3.32 & \footnotesize{17.9M} & \footnotesize{$\geq$5days}
            & 4.06 & \footnotesize{17.4M} &
            &  &  &  \\[-2pt]
        % NeurIPS 2019
        Residual Flow
        ~\cite{chen2019residual}
            % &  &  & 
            & 3.28 & &
            & 4.01 & &
            & 3.76 & & \\[-2pt]
        % NeurIPS 2019
        MaCow
        ~\cite{ma2019macow}
            % &  &  & 
            & 3.16 & \footnotesize{43.5M} &
            &  &  & 
            & 3.69 & \footnotesize{122.5M} & \\[-2pt]
        % NeurIPS 2019
        Neural Spline Flows
        ~\cite{durkan2019spline}
            % &  &  & 
            & 3.38 & \footnotesize{11.8M} &
            & & &
            & 3.82 & \footnotesize{15.6M} & \\[-2pt]
        % ICML 2019
        Flow++
        ~\cite{ho2019flow++}
            % &  &  & 
            & 3.08 & \footnotesize{31.4M} &
            & 3.86  & \footnotesize{169M} &
            & 3.69 & \footnotesize{73.5M} & \\[-2pt]
        % % 2020
        % ANF
        % ~\cite{huang2020augmented}
        %     % &  &  & 
        %     & 3.05 & &
        %     & 3.92 & &
        %     & 3.66 & & \\[-2pt]
        % ICML 2020
        MEF
        ~\cite{xiao2020generative}
            % &  &  & 
            & 3.32 & \footnotesize{37.7M} &
            & 4.05 & \footnotesize{37.7M} &
            & 3.73 & \footnotesize{46.6M} & \\[-2pt]
        % % ICML 2020
        % VFlow
        % ~\cite{chen2020vflow}
        %     % &  &  & 
        %     & 2.98 & 37.8M & 
        %     & 3.83 & & 
        %     & 3.66 &  &   \\[-0pt]
        % % NeurIPS 2020
        % Woodbury NF
        % ~\cite{lu2020woodbury}
        %     % &  &  & 
        %     & 3.47 & & 
        %     & 4.20 & & 
        %     & 3.87 & &  \\[-2pt]
        % % NeurIPS 2020
        % NanoFlow
        % ~\cite{lee2020nanoflow}
        %     % &  & & 
        %     &  3.25 & 10.72M & 
        %     &  &  &  
        %     &  &  &   \\[-2pt]
        % % NeurIPS 2020
        % Convolution Exponential
        % ~\cite{hoogeboom2020flow}
        %     % &  & &
        %     &  3.218 & &
        %     &  &  & 
        %     &  &  &  \\[-2pt]
        % NeurIPS 2020
        Wavelet Flow
        ~\cite{yu2020waveletflow}
            % &  & & 
            &  &  & 
            & 4.08 & \footnotesize{64M} & 
            & 3.78 & \footnotesize{96M} & 822  \\[-2pt]
        % % NeurIPS 2020
        % TayNODE
        % % ~\cite{kelly2020learning}
        %     & 1.039 & & 
        %     & & & 
        %     & & & 
        %     & & &  \\[-2pt]
        % ?? 2021
        DenseFlow
        ~\cite{grcic2021denseflow}
            % &  & & 
            & 2.98 &  & 250
            & 3.63 &  & 310
            & 3.35 &  & 224  \\
        \hline
        \hline
        \multicolumn{10}{|l|}{\textbf{1-Resolution Continuous Normalizing Flow}}\Tstrut \\
        \hline
        % ICLR 2019
        FFJORD
        ~\cite{grathwohl2019ffjord}
            % & 0.99 & &
            & 3.40 & 0.88M & \footnotesize{$\geq$5days}
            & $3.96^{\ddagger}$ & \footnotesize{2.00M}$^{\ddagger}$ & \footnotesize{$>$5days$^{\ddagger}$}
            & x &  & x \\[-0pt]
        % % ICML 2020
        % FFJORD, \textsc{vanilla}
        % % ~\cite{finlay2020train}
        %     % & 0.97 & 68.5 
        %     & 3.36 & & 91.3 
        %     & ?? & ??
        %     & x & x \\
        % ICML 2020
        RNODE
        ~\cite{finlay2020rnode}
            % & 0.97 & 24.4 &
            & 3.38 & 1.36M & 31.84
            & $2.36^{\ddagger}$ & \footnotesize{2.00M} & $30.1^{\ddagger}$
            & $3.83^*$ & \footnotesize{2.00M} & $256.4^*$ \\[-3pt]
            % & 0.97 & 24.4 &
            &  &  & 
            & $3.49^{\mathsection}$ & \footnotesize{1.58M}$^\mathsection$ & $40.39^{\mathsection}$
            & & &  \\
        % NeurIPS 2020
        FFJORD + STEER
        ~\cite{ghosh2020steer}
            % & 0.974 & 51.21 &
            & 3.40 & \footnotesize{1.36M} & 86.34
            & 3.84 & \footnotesize{2.00M} & \footnotesize{$>$5days}
            & & & \\
        % NeurIPS 2020
        RNODE + STEER
        ~\cite{ghosh2020steer}
            & 3.397 & \footnotesize{1.36M} & 22.24
            & 2.35 & \footnotesize{2.00M} & 24.9
            & & & \\[-3pt]
        % Our implementation
            & & & 
            & $3.49^\mathsection$ & \footnotesize{1.58M}$^\mathsection$ & $30.07^\mathsection$
            & & & \\
        \hline
        \hline
        \multicolumn{10}{|l|}{\textbf{\textsc{(Ours)} Multi-Resolution Continuous Normalizing Flow (MRCNF)}}\Tstrut \\
        \hline
        2-resolution MRCNF
            % & ?? & ??
            & 3.65\scriptsize{$\pm$0.62} & \footnotesize{1.34M} & 19.79
            & 3.77\scriptsize{$\pm$0.74}  & \footnotesize{1.34M} & 18.18
            & 3.44\scriptsize{$\pm$0.72} & \footnotesize{2.00M} & 42.30 \\
        2-resolution MRCNF
            % & ?? & ??
            & 3.54\scriptsize{$\pm$0.64}  & \footnotesize{3.34M} & 36.47
            & 3.78\scriptsize{$\pm$0.71}  & \footnotesize{6.68M} & 17.98
            & x & \footnotesize{6.68M} & x \\
        3-resolution MRCNF
            % & ?? & ??
            & 3.79\scriptsize{$\pm$0.60}  & \footnotesize{1.53M} & 17.44
            & 3.97\scriptsize{$\pm$0.70}  & \footnotesize{1.53M} & 13.78
            & 3.55\scriptsize{$\pm$0.71}  & \footnotesize{2.04M} & 35.39 \\
        3-resolution MRCNF
            % & ?? & ??
            & 3.60\scriptsize{$\pm$0.63} & \footnotesize{5.10M} & 38.27
            & 3.93\scriptsize{$\pm$0.71} & \footnotesize{10.19M} & 41.20
            & x & \footnotesize{7.64M} & x \\
        % \multirow{2}{*}{4-resolution MRCNF}
        %     % & ?? & ??
        %     & 3.16 & \footnotesize{1.03M} & 34.18 
        %     &  & \footnotesize{} & 
        %     &  & \footnotesize{} &  \\
            
        %     % & ?? & ??
        %     & 3.27 & \footnotesize{6.85M} & 18.58 
        %     &  & \footnotesize{} & 
        %     &  & \footnotesize{} &  \\
        % 5-resolution MRCNF
        %     % & ?? & ??
        %     & 3.16 & \footnotesize{1.29M} & 32.17 
        %     &  & \footnotesize{} & 
        %     &  & \footnotesize{} &  \\
        \hline
    \end{tabular}
    \label{tab:msflow}
    % \vspace{-1em}
    }
\end{table*}


==> text/table2_ablation.tex <==
\begin{table*}[!htb]
    \small
    \centering
    {\def\arraystretch{1.1}
    \setlength{\tabcolsep}{.15em}   \caption{\normalsize{Ablation study across using Wavelet formulation in \cref{haar} and multi-resolution noise formulation in \ref{subsec:mrnoise}.}}
    \vspace{-.5em}
    \begin{tabular}{|l|ccc|ccc|}
        \hline
        % & \multicolumn{3}{|c|}{MNIST}
        & \multicolumn{3}{c|}{\textbf{\textsc{CIFAR10}}} & \multicolumn{3}{c|}{\textbf{\textsc{ImageNet64}}} \\
        & \textsc{BPD} & \textsc{Param} & \textsc{Time}
        & \textsc{BPD} & \textsc{Param} & \textsc{Time} \\
        % \hline
        % \hline\multicolumn{7}{|l|}{\textbf{Prior relevant methods}}\\
        \hline
        WaveletFlow \cite{yu2020waveletflow}
            % & ?? & ??
            &  &  & 
            & 3.78 & \footnotesize{98.00M} & 822.00 \\
        1-resolution CNF (RNODE) \cite{finlay2020rnode}
            % & ?? & ??
            & 3.38 & \footnotesize{1.36M} & 31.84
            & 3.83 & \footnotesize{2.00M} & 64.10 \\
        \hline\hline
        \multicolumn{7}{|l|}{\textbf{2-resolution}}\\
        \hline
        \cref{haar} WaveletFlow, but with CNFs, w/o multi-res noise
            % & ?? & ??
            & 3.68\scriptsize{$\pm$0.64} & \footnotesize{1.34M} & 27.25
            &  &  &  \\
        \cref{haar} WaveletFlow, but with CNFs, w/ multi-res noise
            % & ?? & ??
            & 3.69\scriptsize{$\pm$0.61} & \footnotesize{1.34M} & 25.88
            & x & \footnotesize{2.00M} & x \\
        \cref{Mdefn} MRCNF w/o multi-res noise
            % & ?? & ??
            & 3.66\scriptsize{$\pm$0.62} & \footnotesize{1.34M} & 19.79
            &  &  &  \\
        \cref{Mdefn} MRCNF w/ multi-res noise \textbf{(Ours)}
            % & ?? & ??
            & 3.65\scriptsize{$\pm$0.62} & \footnotesize{1.34M} & 19.69
            & 3.44\scriptsize{$\pm$0.72} & \footnotesize{2.00M} & 42.30 \\
        \hline\hline
        \multicolumn{7}{|l|}{\textbf{3-resolution}}\\
        \hline
        \cref{haar} WaveletFlow, but with CNFs, w/o multi-res noise
            % & ?? & ??
            & 3.82\scriptsize{$\pm$0.62} & \footnotesize{1.53M} & 22.99
            &  &  &  \\
        \cref{haar} WaveletFlow, but with CNFs, w/ multi-res noise
            % & ?? & ??
            & 3.82\scriptsize{$\pm$0.61} & \footnotesize{1.53M} & 25.28
            & 3.62\scriptsize{$\pm$0.70} & \footnotesize{2.04M} & 43.37 \\
        \cref{Mdefn} MRCNF w/o multi-res noise
            % & ?? & ??
            & 3.79\scriptsize{$\pm$0.62} & \footnotesize{1.53M} & 17.25
            &  &  &  \\
        \cref{Mdefn} MRCNF w/ multi-res noise \textbf{(Ours)}
            % & ?? & ??
            & 3.79\scriptsize{$\pm$0.60} & \footnotesize{1.53M} & 17.44
            & 3.55\scriptsize{$\pm$0.71} & \footnotesize{2.04M} & 35.39 \\
        \hline
    \end{tabular}
    \label{tab:ablation}
    % \vspace{-2.5em}
    }
    \vspace{-1em}
\end{table*}


==> text/table_cifar_full.tex <==
\begin{table}[htb]
    \small
    \centering
    \begin{tabular}{|l@{\hskip 3pt}|@{\hskip 3pt}c@{\hskip 6pt}c@{\hskip 6pt}c@{\hskip 3pt}|@{\hskip 3pt}c@{\hskip 3pt}|@{\hskip 3pt}c@{\hskip 6pt}c@{\hskip 3pt}|}
        \hline
        \textbf{\textsc{CIFAR10}} & \textsc{Param}
        % & \multicolumn{3}{|c|}{MNIST}
        % & \multicolumn{5}{|c|}{CIFAR 10}
        % & \multicolumn{3}{|c|}{ImageNet64} 
        % \\
        % \cline{3-7} 
        % &
        % & \begin{tabular}{@{}c@{}}Train \\ BPD\end{tabular} 
        & \textsc{BPD}
        % & \begin{tabular}{@{}c@{}}Time \\ (Hours)\end{tabular}
        & \textsc{Time}
        & \textsc{FID} 
        % & \begin{tabular}{@{}c@{}}SVHN \\ Train\end{tabular} 
        & \textsc{SVHN} 
        & \textsc{TIN}
        \\
        \hline
        \hline
        \multicolumn{7}{|l|}{\textbf{(FFJORD) 1-resolution Continuous Normalizing Flow}~\cite{grathwohl2019ffjord}} \\
        \hline
        % ICLR 2019
        1res F
        % ~\cite{grathwohl2019ffjord}
            & \multirow{4}{*}{\footnotesize{0.16M$^*$}}
            &  3.40 & \footnotesize{$\geq$5days} &  &  &
            \\[-1pt]
        % ICML 2020
        1res F R
        % ~\cite{finlay2020rnode}
            &
            & 3.38 & 31.84 & \footnotesize{139.70$^\ddagger$} & \footnotesize{2.21$^\ddagger$} & \footnotesize{3.33$^\ddagger$}
            \\[-1pt]
        % NeurIPS 2020
        1res F + S
        % ~\cite{ghosh2020steer}
            &
            & 3.40 & 86.34 & \footnotesize{152.60$^\ddagger$} & \footnotesize{2.29$^\ddagger$} & \footnotesize{3.44$^\ddagger$}
            \\[-1pt]
        % NeurIPS 2020
        1res F R + S
        % ~\cite{ghosh2020steer}
            &
            & 3.397 & 22.24 & \footnotesize{148.77$^\ddagger$} & \footnotesize{2.24$^\ddagger$} & \footnotesize{3.38$^\ddagger$}
            \\
        \hline
        1res F R
            & \footnotesize{0.24M$^\ddagger$}
            & \footnotesize{3.35$^\ddagger$} & \footnotesize{26.73$^\ddagger$} & \footnotesize{138.82$^\ddagger$} & \footnotesize{2.19$^\ddagger$} & \footnotesize{3.30$^\ddagger$}
            \\
        % \hline
        % 1res F R
        %     & \footnotesize{0.32M}
        %     & 3.34 & 16.86 & 135.96 & 2.20 & 3.30
        %     \\
        \hline
        1res F R
            & \footnotesize{0.40M$^\ddagger$}
            & \footnotesize{3.32$^\ddagger$} & \footnotesize{25.88$^\ddagger$} & \footnotesize{132.60$^\ddagger$} & \footnotesize{2.18$^\ddagger$} & \footnotesize{3.28$^\ddagger$}
            \\
        \hline
        % 2 resolutionS
        \hline
        \multicolumn{7}{|l|}{\textbf{\textsc{(Ours)} 2-res MRCNF}}\\
        \hline
        % 2res F
        %     & \multirow{4}{*}{\footnotesize{0.08M}}
        %     & 2.14 & 15.94 & 114.43 & 0.57 & 2.10
        %     \\
        2res F R
            & \footnotesize{0.09M}
            & 2.00 & 14.97 & 107.30 & 0.49 & 1.97
            \\
        % 2res F + S
        %     &
        %     & 2.06 & 24.32 & 110.25 & 0.52 & 2.02
        %     \\
        % 2res F R + S
        %     &
        %     & 2.05 & 12.45 & 107.99 & 0.51 & 2.01
        %     \\
        \hline
        2res F
            & \multirow{4}{*}{\footnotesize{0.16M}}
            &  1.87 & 17.43 & 99.69 & 0.44 & 1.84
            \\[-1pt]
        2res F R
            &
            &  1.80 & 17.22 & 103.52 & 0.38 & 1.77
            \\[-1pt]
        2res F + S
            &
            &  2.14 & 17.71 & 102.29 & 0.58 & 2.08
            \\[-1pt]
        2res F R + S
            &
            & 1.94 & 14.81 & 104.13 & 0.51 & 1.93
            \\
        \hline
        2res F
            & \multirow{4}{*}{\footnotesize{0.32M}}
            & 1.85 & 17.89 & 97.96 & 0.73 & %11.98
            \\[-1pt]
        2res F R
            &
            & 1.69 & 16.37 & 93.38 & 0.31 & 1.63
            \\[-1pt]
        2res F + S
            &
            & 2.04 & 18.76 & 121.58 & 0.50 & 1.99
            \\[-1pt]
        2res F R + S
            &
            & 1.74 & 18.43 & 100.78 & 0.32 & 1.70
            \\
        \hline
        2res F R
            & \footnotesize{0.48M}
            & \textbf{1.59} & 24.76 & \textbf{88.52} & 0.25 & 1.52
            \\
        \hline
        2res F R
            & \footnotesize{0.64M}
            & 1.61 & 22.85 & 89.55 & 0.25 & 1.53
            \\
        \hline
        2res F R
            & \footnotesize{0.80M}
            & 1.62 & 22.36 & 88.40 & 0.29 & 1.60
            \\
        \hline
        % 3 resolutionS
        \hline
        \multicolumn{7}{|l|}{\textbf{\textsc{(Ours)} 3-res MRCNF}}\\
        \hline
        3res F
            & \multirow{4}{*}{\footnotesize{0.13M}}
            & 1.76 & 19.83 & 110.86 & 0.16 & 1.70
            \\[-1pt]
        3res F R
            &
            & 1.70 & 19.68 & 106.32 & 0.16 & 1.67
            \\[-1pt]
        3res F + S
            &
            & 2.02 & 22.57 & 105.24 & 0.39 & 2.02
            \\[-1pt]
        3res F R + S
            &
            & 1.72 & 19.97 & 103.92 & 0.18 & 1.72
            \\
        \hline
        3res F
            & \multirow{4}{*}{\footnotesize{0.48M}}
            & 1.54 & 21.51 & 91.80 & 0.06 & 1.46
            \\[-1pt]
        3res F R
            &
            & 1.32 & 21.48 & 91.82 & 0.00 & 1.33
            \\[-1pt]
        3res F + S
            &
            & 1.72 & 21.09 & 104.08 & 0.27 & 1.70
            \\[-1pt]
        3res F R + S
            &
            & 1.44 & 23.44 & 95.21 & 0.03 & 1.41
            \\
        \hline
        3res F R
            & \footnotesize{0.72M}
            & \textbf{1.28} & 21.04 & \textbf{88.51} & -0.14 & 1.23
            \\
        \hline
        3res F R
            & \footnotesize{0.96M}
            & 1.34 & 21.84 & 88.99 & -0.02 & 1.29
            \\
        \hline
        3res F R
            & \footnotesize{1.20M}
            & 1.32 & 20.73 & 91.24 & -0.12 & 1.28
            \\
        \hline
        % 4 resolutionS
        \hline
        \multicolumn{7}{|l|}{\textbf{\textsc{(Ours)} 4-res MRCNF}}\\
        \hline
        % 4res F
        %     & \multirow{4}{*}{\footnotesize{0.09M}}
        %     & 2.00 & 13.58 & 121.27 & 0.38 & 1.95
        %     \\
        4res F R
            & \footnotesize{0.09M}
            & 2.02 & 9.86  & 122.16 & 0.40 & 1.97
            \\
        % 4res F + S
        %     &
        %     & 2.11 & 13.28 & 128.78 & 0.52 & 2.07
        %     \\
        % 4res F R + S
        %     &
        %     & 2.02 & 10.33 & 122.19 & 0.50 & 1.99
        %     \\
        \hline
        4res F
            & \multirow{4}{*}{\footnotesize{0.17M}}
            & 1.77 & 19.89 & 119.34 & 0.43 & 1.80
            \\[-1pt]
        4res F R
            &
            & 1.56 & 15.74 & 107.11 & 0.08 & 1.50
            \\[-1pt]
        4res F + S
            &
            & 1.86 & 18.01 & 111.37 & 0.25 & 1.76
            \\[-1pt]
        4res F R + S
            &
            & 1.65 & 17.58 & 117.64 & 0.13 & 1.58
            \\
        \hline
        4res F
            & \multirow{4}{*}{\footnotesize{0.64M}}
            & 1.42 & 19.95 & 93.89 & -0.01 & 1.44
            \\[-1pt]
        4res F R
            &
            & \textbf{1.28} & 19.08 & \textbf{92.19} & -0.14 & 1.22
            \\[-1pt]
        4res F + S
            &
            & 1.88 & 17.73 & 98.24 & 0.2 & 1.78
            \\[-1pt]
        4res F R + S
            &
            & 1.44 & 17.60 & 109.68 & -0.04 & 1.39
            \\
        \hline
        \hline
        \multicolumn{7}{|l|}{\textbf{\textsc{(Ours)} 5-res MRCNF}}\\
        \hline
        5res F R
            & \footnotesize{0.81M}
            & \textbf{1.28} & 19.42 & \textbf{99.98} & -0.15 & 1.21 \\
        \hline
        \hline
        \multicolumn{7}{|l|}{\textbf{\textsc{(Ours)} 6-res MRCNF}}\\
        \hline
        6res F R
            & \footnotesize{0.97M}
            & \textbf{1.24} & 20.52 & \textbf{107.83} & -0.19 & 1.18 \\
        \hline
    \end{tabular}
    \caption{\small{Metrics of \gls{msflow-image} models trained on CIFAR10 (lower is better in all cases): number of parameters, average \gls{bpd} of CIFAR10 Val images, time in hours, FID, average \gls{bpd} of SVHN Test and TinyImageNet Test (TIN) images. F=FFJORD~\cite{grathwohl2019ffjord}, R=RNODE~\cite{finlay2020rnode}, S=STEER~\cite{ghosh2020steer}. $^*$Number of parameters used in model to reproduce results. $^\ddagger$Unreported in original paper, computed by us.}}
    \label{tab:msflow_cifar}
    % \vspace{-1.5em}
\end{table}

